Travel Cost Calibration for Multi-Agent Target Assignment and Pathfinding

Target assignment and pathfinding (TAPF) is an appealing extension of classical multi-agent pathfinding (MAPF): each agent has a set of targets, and the planner must both assign a target to each agent and plan collision-free paths for them. A trivial approach is to compute an assignment that minimizes the total single-agent shortest-path distance over agent--target pairs, and then solve the resulting MAPF instance. However, this approach falls short because the shortest-path distance remains a proxy that ignores interference among agents. Assigning targets based on the costs agents actually pay, which depend on how every other agent is assigned and routed, would yield a better final outcome. To this end, we propose an iterative TAPF method that improves target assignments by calibrating travel cost estimates from fast, suboptimal MAPF feedback. Experiments show that our method produces solutions close to optimal on small instances and outperforms existing planners in solution quality on larger ones.

==> fig/init.tex <==
  \begin{figure}[t!]
      \begin{minipage}[c]{1\columnwidth}
          \centering
          \includegraphics[width=0.8\linewidth]{fig/raw/init_runtime_lak303d_n800.pdf}
      \end{minipage}
      \caption{
      Comparison with different initial target assignment methods.
      }
      \label{fig:init}
\end{figure}

==> table/experiment.tex <==
\begin{table}[t]
    \centering
    \label{tab:scenario_params}
    \begin{tabular}{lrrrrr}
        \toprule
        & & \multicolumn{4}{c}{$r$} \\
        \cmidrule(lr){3-6}
        Map & $d$ & \multicolumn{4}{c}{$n = 50 / 100 / 150 / 200$} \\
        \midrule
        \mapname{maze-32-32-4}           & 40  & 8 & 14 & 18 & 22 \\
        \midrule
        & & \multicolumn{4}{c}{$n = 200 / 400 / 600 / 800$} \\
        \midrule
        \mapname{random-64-64-20}        & 43  & 20 & 35 & 45 & 55 \\
        \mapname{warehouse-10-20-10-2-1} & 76  & 16 & 26 & 36 & 45 \\
        \mapname{ost003d}                & 143 & 20 & 30 & 45 & 60 \\
        \mapname{warehouse-20-40-10-2-1} & 154 & 21 & 32 & 41 & 48 \\
        \mapname{lak303d}                & 173 & 30 & 45 & 55 & 60 \\
        \mapname{Paris-1-256}            & 183 & 19 & 30 & 39 & 48 \\
        \mapname{den520d}                & 187 & 50 & 55 & 70 & 85 \\
        \bottomrule
    \end{tabular}
    \caption{Scenario parameters per map: the distance $d$ of \scenEqdist
    and the hotspot radius $r$ of \scenHotspot per number of agents $n$.}
    \label{tab:experiment}
\end{table}
